Metric-agnostic Ranking Optimization

Ranking is at the core of Information Retrieval. Classic ranking optimization studies often treat ranking as a sorting problem with the assumption that the best performance of ranking would be achieved if we rank items according to their individual utility. Accordingly, considerable ranking metrics have been developed and learning-to-rank algorithms that have been designed to optimize these simple performance metrics have been widely used in modern IR systems. As applications evolve, however, people's need for information retrieval have shifted from simply retrieving relevant documents to more advanced information services that satisfy their complex working and entertainment needs. Thus, more complicated and user-centric objectives such as user satisfaction and engagement have been adopted to evaluate modern IR systems today. Those objectives, unfortunately, are difficult to be optimized under existing learning-to-rank frameworks as they are subject to great variance and complicated structures that cannot be explicitly explained or formulated with math equations like those simple performance metrics. This leads to the following research question -- how to optimize result ranking for complex ranking metrics without knowing their internal structures? To address this question, we conduct formal analysis on the limitation of existing ranking optimization techniques and describe three research tasks in \textit{Metric-agnostic Ranking Optimization}. Through the discussion of potential solutions to these tasks, we hope to encourage more people to look into the problem of ranking optimization in complex search and recommendation scenarios.

==> sec-evaluation.tex <==
\vspace{-3ex}
\section{Evaluation, Management, and Expected Results}
\label{sec:eval}
\vspace{-3ex}
\vspace{-1ex}

\subsection{Platform and Datasets}. 
The proposed research will be conducted on multiple ranking tasks in IR include Web search, product search, etc. 
We have already obtained the access of multiple real-world ranking and retrieval datasets such as MSLR~\cite{MSletor}, Yahoo!~\cite{Yahooletor}, Istella~\cite{istella}, Amazon transactions~\cite{amazon}, MSMARCO~\cite{MSMARCO}.
We have also partnered with our colleagues in industry for potential experiments on real-world IR systems in future (support letter attached).
For computing support, we will develop and test the proposed techniques with the Center for High Performance Computing in University of Utah. 
%task
%dataset
%resources

\vspace{-1ex}
\subsection{Evaluation Plan}. 
The evaluation of proposed research will be conducted with both offline simulations and online experiments.
Offline simulation helps us efficiently develop and test the proposed techniques without extensive demand on online user data.
For example, on public learning-to-rank datasets~\cite{MSletor,Yahooletor,istella}, we can compute standard ranking metrics such as ERR~\cite{chapelle2009expected} and NDCG~\cite{jarvelin2002cumulated} with the relevance labels in the datasets but retain these fine-grained information from ranking models and only make the final metric scores on each ranking available for training processes.
Through this way, we can simulate metric-agnostic ranking scenarios where we can access the performance of each ranking but have no clue on the structure of the metrics.
Online experiments focus on testing the true effectiveness of proposed algorithms in real-world applications.
By collaborating with our colleagues in industry, we plan to collect real user interaction data with real search traffic for the training of proposed methods.
The final evaluation will be conducted with standard industrial pipelines such as online A/B testing.
 

% simluation and online
% simulation process
% online process

\vspace{-1ex}
\subsection{Management Plan}. 
%project plan
This is three-year project that will involve two students advised by the PI. 
In Year 1\&2, the first student will focus on Task 1 and develop effective approaches to build surrogate models for structure-agnostic ranking metrics.
In the meantime, the second student will work on Task 2 and study potential solutions for optimizing ranking models in metric-agnostic scenarios with the help of public learning-to-rank datasets and offline simulation experiment platforms.
In Year 3, both students will collaborate to develop efficient parameter optimization and exploration methods for Task 3 by combining the surrogate models in Task 1 with optimization techniques in Task 2.
Also, we will explore the possibility of applying proposed research to real-world IR systems in Year 3 through our partnership with industry researchers and student summer internships.
All benchmark datasets and evaluation frameworks will be published and shared with the community to boost future research.
%In Year 1, the PI and student 1 will focus on Task 1 and develop model-intrinsic approaches for explainable search on standard e-commerce search and recommendation datasets. 
%In Year 2, with existing studies on explainable IR and the results from Year 1, two new students will be recruited to work on the model-agnostic approaches for post-hoc search explanations and the development of comparison-based crowdsourcing platforms for explanation evaluations. 
%In the meantime, student 1 will move to more general search scenarios including web search and interactive information retrieval. 
%In Year 3, student 1, 2, and 3 will collaborate to compare the effectiveness of search explanations generated by model-intrinsic approaches (i.e., pre-hoc explanations) and model-agnostic approaches (i.e., post-hoc explanations). 
%Also, we will construct benchmark datasets and offline explanation evaluation metrics accordingly and share with the community to boost the future research on this topic. Throughout the projects, both PIs will closely supervise and collaborate with the students for research and development.

\vspace{-1ex}
\subsection{Expected Results}. 
% contribution again
We expect the proposed research will lead to the development of new theories and techniques on ranking optimization, especially for the optimization of complex ranking metrics.
Specifically, the outcomes of this research will include 1) multiple methods to resolve noise/variance and build surrogate models for complex ranking metrics; 2) new paradigms for ranking problem formulation and a series of algorithms for differentiable ranking optimization; and 3) a couple of empirical efficient and effective methods to incorporate the optimization of structure-agnostic ranking metrics into real-world IR applications.
This research will lead to publications in top-tier conferences or journals as well as open-source packages and benchmark collections that will be shared to the community.

%We expect the developed techniques will improve both the retrieval effectiveness and the explainability of information retrieval systems. Specifically, the outcomes of this research will include 1) multiple retrieval models and design paradigms with intrinsic explainability and scrutable ranking functions; 2) a set of post-hoc analytic and simulative frameworks that can mimic and explain the behavior of an arbitrary IR system; and 3) a series of offline performance metrics and benchmark datasets for evaluation and a guideline on how to choose different approaches for explainable IR in practice. This research will lead to publications in top-tier conferences or journals as well as open- source software packages and benchmark collections that will be shared to the community.


==> sec-research.tex <==
%!TEX root=sigir2023.tex
\section{Overview}
\label{sec-research}

In order to conduct metric-agnostic ranking optimization 


\textit{Structure-agnostic metric modeling and simulation}. 
Complex ranking metrics such as user engagement are usually collected in online services or contain hidden factors that cannot be modeled and computed for ranking systems offline.
However, due to the significant cost of online experiments, it is often infeasible to collect metric scores for a large set of possible rankings, which essentially limits the size of training data for learning to rank and harm the generalizability of optimization algorithms. 
In this research, we tackle the data sparsity problem for structure-agnostic ranking metrics from three directions: 1) modeling and calibrating metric scores to reduce noise and variance; 2) constructing surrogate models for offline metric computation based on local context; and 3) designing and evaluating off-policy learning algorithms for surrogate models to enhance generalizability. 
Our goal is to develop accurate and robust knowledge distillation techniques and offline surrogate models for complex ranking metrics without extensive online experiments.
	
	
	% motivation
	% question
	% what we do
	% what we can achieve
	%stata
	%through effective, they cannot answer
	%In this research task
	%the future of self-explain
	
\textit{Differentiable ranking process with coarse-grained reward}. 
Complex ranking metrics are often defined on list level, which means that a metric score can only be obtained over a full ranking of result candidates. 
Without the PRP assumption, we cannot simplify ranking as a sorting problem in which the theoretical performance bound on list level can be guaranteed by correctly predicting the partial orders of item pairs.
This means that existing ranking optimization techniques based on partial order predictions are not applicable.
In this research, we propose to reformulate ranking as a sampling problem and construct stochastic ranking algorithms by modeling the generation of a result ranking with probabilistic frameworks. By applying different probabilistic sampling strategies, we smooth the discrete reward computed with complex ranking metrics and make the whole ranking optimization process differentiable in parameter space.
	
	
\textit{Efficient ranking exploration in parameter space}. 
Even with surrogate ranking metrics and differentiable optimization frameworks, ranking is still considered to be a difficult task in both IR and ML communities because of its unique and vast parameter space (e.g., the possible ranking of $n$ items is $O(n!)$). 
State-of-the-art ranking optimization algorithms usually simplify the parameter space under the PRP framework by decomposing ranking problems as partial order predictions and constructing uni-variate scoring functions that only score one candidate a time.
This, however, is no longer feasible in metric-agnostic ranking optimization because complex ranking metrics don't follow PRP.
In this research, we design new techniques to conduct efficient ranking exploration in parameter space without the PRP assumption.
We plan to develop new algorithms for ranking sampling and multi-objective optimization that guide ranking models to explore parameter space effectively with less training steps and model updates. 
